Ethics Testing: Proactive Identification of Generative AI System Harms

Generative Artificial Intelligence (GAI) systems that can automatically generate content in the form of source code or other contents (e.g., images) has seen increasing popularity due to the emergence of tools such as ChatGPT which rely on Large Language Models (LLMs). Misuse of the automatically generated content can incur serious consequences due to potential harms in the generated content. Despite the importance of ensuring the quality of automatically generated content, there is little to no approach that can systematically generate tests for identifying software harms in the content generated by these GAI systems. In this article, we introduce the novel concept of ethics testing which aims to systematically generate tests for identifying software harms. Different from existing testing methodologies (e.g., fairness testing that aims to identifying software discrimination), ethics testing aims to systematically detect software harms that could be induced due to unethical behavior (e.g., harmful behavior or behavior that violates intellectual property rights) in automatically generated content. We introduced the concept of ethics testing, discussed the challenges therewithin, and conducted five case studies to show how ethics testing can be performed for generative AI systems.

==> datasettable.tex <==
\begin{table*}[h]
\caption{Datasets for Code Generation}
\label{tab:dataset}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{3cm}|}
\hline
\small
Benchmark &
  Natural Languages &
  Programming Languages &
  Supported Tasks &
  Size &
  Test case &
Unique Features \\ \hline
APPS~\cite{hendrycks2021measuring} &
  English &
  Python &
  Text-code &
  10,000 problems &
  130,000 total test cases &
  One of the earlier dataset with crowd-sourced   questions for program synthesis \\ \hline
HumanEval~\cite{chen2021evaluating} &
  English &
  Python &
  Text-code &
  164 problems &
  Average 7.7 tests per problem &
  Handwritten problems to evaluate   functional correctness and measure problem-solving capabilities \\ \hline
MBPP~\cite{austin2021program} &
  English &
  Python &
  Text-code &
  974 python functions &
  3 test cases for each problem &
  Measure the ability of these models to   synthesize short Python programs \\ \hline
CONCODE~\cite{iyer2018mapping} &
  English &
  Java &
  Text-code &
  100,000   (classes, NL, code) tuples &
  No test &
  Classes from diverse domains\\ \hline
PandasEval, NumpyEval~\cite{zan2022cert} &
  English &
  Python &
  Text-code &
  101 programming problems &
  20 tests for each problem &
  Library-oriented code generation \\ \hline
%CODEXGLUE~\cite{DBLP:journals/corr/abs-2102-04664} &  English &  6 languages & 10 tasks &  113 programming tasks from recent contests, 335 incorrect   solutions &  1-3 public tests for each problem &   Collection of datasets that supports 10 programming language understanding and generation tasks.\\ \hline
MCoNaLa~\cite{wang2022mconala} &
  Spanish, Japanese, and Russian &
  Python &
  Text-code & 
  896 NL-Code pairs & No test
   &
  Support several natural languages beyond English \\ \hline
LLMDefects~\cite{fan2023automated} &
  English &
  Java &
  Text\&code-code &
  113 programming tasks from recent contests, 335 incorrect   solutions &
  1-3 public tests for each problem &
  Contains mistakes in code generated by LLMs.\\ \hline
ClassEval~\cite{du2023classeval} &
  English &
  Python &
  Text-code &
  100 tasks &
  Contain method-level and class-level   tests &
  Class-level code generation \\ \hline
AixBench~\cite{hao2022aixbench} &
  English, Chinese &
  Java &
  Text-code &
  175 samples for automated Test, 161 NL   Task Description &
  Contain hand-crafted tests &
  Contain hand-crafted automated test   cases \\ \hline
  MultiPL-E~\cite{multiple} &
  English &
  19 languages (e.g., Julia, Swift) &
  Text-code &
  161 problems from HumanEval~\cite{chen2021evaluating}, 974 from MBPP~\cite{austin2021program}  &
  Use tests from prior benchmarks~\cite{chen2021evaluating,austin2021program} &
  Extend HumanEval~\cite{chen2021evaluating} and
MBPP~\cite{austin2021program} to 18 languages by translating programs and unit tests\\ \hline
SWE-Bench~\cite{jimenez2023swe} &
  English &
  Python &
  Text\&code-code&
  2294 problems from 12 projects &
  Average 120.8 total tests for each problem &
  Evaluate the ability to resolve real-world GitHub\\ \hline
CodeScope~\cite{yan2023codescope} &
  English &
  43 languages &
  8 tasks&
  200--5,382 samples for each task &
  Contain tests for some tasks &
  Evaluate generated code on difficulty, efficiency,
and length\\ \hline
NoFunEval~\cite{singhal2024nofuneval} &
  English &
  Python, Java, C, JavaScript, Kotlin&
  Text\&code-code, classify correctness &
  47--397 samples for each task &
  No test &
  Evaluate non-functional requirements (latency, security, efficiency)\\ \hline
LiveCodeBench~\cite{jain2024livecodebench} &
  English &
  Python &
  Text\&code-code &
  Collect new problems over time &
  Use tests from programming problems or LLM-generated tests &
  Mitigate contamination issues by crawling new problems\\ \hline
\end{tabular}}
\end{table*}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> others.tex <==
\begin{lstlisting}[style=mystyle, escapechar=^,caption=Crash due to transformation issue when joining variable declaration in Eclipse 4.7.1, upquote=true, label={lst:transformation}]
/**
     * ChatGPT generated method to convert to string
     * @param throwable
     * @return 
     */
    private static String convertStackTraceToString(Throwable throwable) {
        StringBuilder result = new StringBuilder();

        // Append the exception message (if any)
        if (throwable.getMessage() != null) {
    result.append(throwable.getClass().getName()).append(": ").append(throwable.getMessage());
            result.append(System.lineSeparator());
        } else {        
    result.append(throwable.getClass().getName()).append(System.lineSeparator());
        }

        // Append each stack trace element
        for (StackTraceElement element : throwable.getStackTrace()) {
            result.append("\tat ").append(element.toString()).append(System.lineSeparator());
        }

        // Append the cause (if any)
        Throwable cause = throwable.getCause();
        if (cause != null) {
            result.append("Caused by: ").append(convertStackTraceToString(cause));
        }
        return result.toString();
    }
}
\end{lstlisting}

==> sec1-old.tex <==
\section{Introduction}
Generative Artificial intelligence (GAI) systems, which automate the decision-making process and generation of new content, is penetrating every public sector and industry. The importance of ethical use of software in automated decision-making is highlighted in Treasury Board Directive on Automated Decision-Making by
the Government of Canada~\cite{automateddecision}. Meanwhile, worldwide authorities from different disciplines are recognizing the potential risks posed by AI-powered software by publishing guiding principles and code of conducts for organizations developing AI systems, including UNESCO's first-ever global standard on AI ethics – the ``Recommendation on the Ethics of Artificial Intelligence''~\cite{unesco},
%the\cite{commision}, 
the October 2023 Global Privacy Assembly resolution on GAI systems~\cite{globalassembly}, and the June 2024 G7 Leaders Statement~\cite{gseven}. To build a digital society where technological innovation is socially-beneficial and human dignity is in safe hand, ensuring that automatically generated content is ethical has become a global concern.

%The growing importance of open-source governance is highlighted in several Canadian directives, including Government of Canada Digital Standards, Public Service Commission of Canada’s fourth Open Government Implementation Plan with the vision of shifting Canadian government to an ``open approach''. 

%\todo{Remove this paragraph?}This project brings together experts in ethics, data quality, and software testing to close the ethics gaps in software testing. We will apply ethical principles, data quality assurance methodologies, and test generation techniques to design actionable guidelines, and develop automated testing framework for identifying ethical issues in software, ensuring that automatically generated content will not cause harms to society, and adhere to the code of conducts. 
%open source governance, closing the ethic gaps in open source governance and practices. We will apply ethical principles and machine learning techniques to design actionable guidelines, and develop  state-of-the-art decision support tools for detecting and preventing ethical problems in open source community, started by provoking a reassessment of ethics in open lens (refer to as \emph{open ethics} in this project). Open ethics is applied ethics that focuses on real-world situations in which open source contributions of diverse forms (e.g., human discussion, data, software) occur. %-- How should we apply ethical principles and values to the way we contribute to open source?
%As noted in Treasury Board of Canada Secretariat's ``Open First Whitepaper''~\cite{whitepaper}, ``open organizations are communal'', studying ethics in the open lens will help to understand how individuals from diverse backgrounds and cultures communicate and contribute under the communal respect principle. The wealth of open data presents numerous opportunities to apply machine learning techniques to augment current modeling with data-driven recommendations and guidance.  


%An analogy is the predictive typing that occurs on cell phones and word processors [2], [3] and the auto-completion feature embedded in many of the integrated development environments (IDEs) to predict the next code token (e.g. a letter, or a function call) to save software engineers’ effort [4]–[7]; in our case, the trained model, via a design assistant, will predict the next step in the CAD process based on the sequence that led to the current point. 

 %As emphasized in the ``Open First Whitepaper'', the important next steps in shifting the Government of Canada to the open approach include open standards, the open source software contribution, and open source community building.
%A key component that drives the automated generation of content is the availability and the use of open data. 
%While extensive recent work has been done on detecting common types of ethical issues (e.g., fairness\todo{cite?}) in AI systems, little progress has been made on generation of unethical content such as harmful content or content that violates intellectual property rights. These aspects have the potential to unlock important and immediately applicable insight towards improving the quality of automatically generated content which is currently limited by lack of best practice and systematic detection.  
%The growing importance of open-source software is highlighted in several Canadian directives, including Government of Canada Digital Standards, Public Service Commission of Canada’s fourth Open Government Implementation Plan, and the ``Open First Whitepaper''~\cite{whitepaper} by Treasury Board of Canada Secretariat. As emphasized in the ``Open First Whitepaper'', the important next steps in shifting the Government of Canada to the open approach include open standards, the open-source software contribution, and open-source community building. %that draft how to shift government to an “Open” approach.  
%With the increasing popularity of 

%GitHub being one of the most popular open-source development platforms, 


%Problems related to ethics have become an important yet often neglected topic. 
%It does! “Work in the open by default” is one of the Government of Canada Digital Standards. Appendix A to the new Directive on Service and Digital says, “where possible, use open standards and open source software first” (section A.2.3.8.1), and “by default any source The Treasury Board of Canada Secretariat has written this whitepaper to pull together our thinking on how to shift government to an “Open” approach. code written by the government must be released in an open format” (section A.2.3.8.3). Our colleagues in the Office of the CIO have published detailed guidance on open source,
%The Treasury Board of Canada Secretariat has written this whitepaper to pull together our thinking on how to shift government to an “Open” approach. 

%As we continue to move towards a more open government and an engaged citizenry, we still rely heavily on proprietary technologies and standards for our core operations and programs. This leads to an important question: How can the Government of Canada more broadly adopt open source software and open standards in its development of tools and solutions?
%Public Service Commission of Canada’s (PSC) fourth Open Government Implementation Plan (OGIP
%Government of Canada~\cite{whitepaper}
%With the increasing popularity of open-source development in platforms like GitHub, problems related to ethics have become an important yet often neglected topic. 

Existing literature mostly focus on common problems such as fairness testing for identifying software discrimination across different gender, ages, and races~\cite{chen2024fairness, dehal2024exposing,galhotra2017fairness,udeshi2018automated}. %when investigating ethical issues in open source projects. 
Despite the ``Proportionality and Do No Harm'' principle being listed before ``Fairness'' in UNESCO’s ``Recommendation on the
Ethics of Artificial Intelligence'', we observe that the focus on fairness issues lead to a general tendency to neglect other important ethical issues such as software harms. %and yet there are rarely any testing technique that aims to systematically identify harmful contents. %At one extreme, even in the so-called \emph{Data Ethics Framework} by the United Kingdom Government~\footnote{https://www.gov.uk/government/publications/data-ethics-framework/data-ethics-framework-2020} where ``ethics'' is part of the name, only three principles (transparency, accountability, and fairness) have been included. 
Indeed, 
little progress has been made on the generation of unethical content such as harmful content or content that violates intellectual property rights. These aspects have the potential to unlock important and immediately applicable insight towards improving the quality of automatically generated content which is currently limited by lack of understanding of unethical issues and systematic detection.
%Identifying other ethical issues, especially related to the use of open data is not well-understood, given that it lies at the interdisciplinary intersection of applied ethics, open data governance, and software testing. Correspondingly, the current practices including code of ethics and ethical considerations in open source ~\cite{gotterbarn1997software,hall2001ethical,singer2002ethical,vinson2001getting} are designed based on examples and studies in other disciplines (e.g., politics). 
%A prominent example of ethical problems in open source is an incident in Linux, a well-known open-source software (OSS) project, where researchers investigated the feasibility of introducing vulnerabilities in OSS by making \emph{hypocrite commits} (commits that deliberately introduce critical vulnerabilities)~\cite{wu2021feasibility}. The Linux developers claimed that making ``hypocrite commits'' is ``not ethical'' as it wasted developers' time in reviewing invalid patches. This incident has revealed an attack on the basic premise of open source contribute itself (i.e., anyone can contribute and any OSS is susceptible to similar incidents). 
%However, our recent study~\cite{win2023towards} revealed that there remains many unexplored unethical behavior that can exploit open-source data. For example, when naming a software artifact (e.g., a product name), open-source developers may incur unethical behavior such as \emph{naming confusion} (i.e., selecting a name which has a conflict of interest with other organization or individuals) or \emph{offensive language} (e.g., selecting unethical product names like ``Scroll of Genocide'' that promote mass-murder). 
One research direction is represented by proposing new regulations to address harmful content online. For example, the Government of Canada has 
proposed a framework to potentially implement new legislation and rules to consider harmful content~\cite{harmful}. 
Such regulations can provide guidelines for practitioners to pay attention to potential unethical content.
However, to ensure compliance and help practitioners control the ethics of the generated content, systematic testing for unethical content is essential, especially with the growing volume and variety of the generated content and the increasing reliance on them. 
%With the increasing reliance on automatically generated content, systematically identifying unethical behavior in these generated content is essential and yet challenging.

In this work, we first discuss the challenges of ethics testing, such as the lack of understanding due to the interdisciplinary nature and the lack of quality measurement methods. Then, we formally define ethics testing, which is interdisciplinary domain across software engineering and social science. Furthermore, we propose a framework for systematic ethics testing, and perform preliminary case studies to demonstrate the feasibility and effectiveness of the framework. Our case study results provide evidence that new ethics testing methodology that injects unethical behavior into prompts given to generative AI systems can induce these systems to generate unethical content even without providing any warning to indicate the misuse of the AI systems.

\section{Challenges in Ethics Testing}
\label{sec:cha}
In this section, we discuss three main challenges that hinder the wide adoption of ethics testing. 

\noindent\textbf{Challenge 1: Lack of understanding due to the interdisciplinary nature of ethics testing.} Ethics testing is a multidimensional problem given that it lies at the interdisciplinary intersection of applied ethics, human-computer interaction, open data governance, and software testing. In software engineering, the current practices include code of ethics and ethical considerations in open source ~\cite{gotterbarn1997software,hall2001ethical,singer2002ethical,vinson2001getting}. % are designed based on examples and studies in other disciplines (e.g., %empirical studies, software engineering research). 
Other domains include their own understanding of ethics (e.g., AI~\cite{jobin2019global} or social science~\cite{plinio2010state}).
Aligning such understandings and gathering requirements for ethics testing of intelligent systems is important yet challenging.

\noindent\textbf{Challenge 2: Lack of quality measurement on ethics.} The key underlying problem in ethics testing lies in the fact that ethics is not included in traditional quality metrics. For example, in traditional quality characteristics specified in ISO/IEC 25010, only eight quality characteristics are included: (1) functional suitability, (2) performance efficiency, (3) compatibility, (4) usability, (5) reliability, (6) security, (7) maintainability, and (8) portability. All the eight quality characteristics are loosely connected with the concept of ethics. Indeed, even in the \emph{Data Ethics Framework} designed by the United Kingdom Government~\footnote{https://www.gov.uk/government/publications/data-ethics-framework/data-ethics-framework-2020} where ``ethics'' is part of the name of the framework, important ethical principles (e.g., ``do not harm'') have not been carefully considered where
only three overarching principles (transparency, accountability, and fairness) have been included, requesting each principle to be measured with a score  from 0 to 5 where a score of 5 representing full compliance to the principle. With extensive prior literature focusing mostly on discussing responsible use of AI in terms of fairness~\cite{chen2024fairness, dehal2024exposing,galhotra2017fairness,udeshi2018automated}, there is a \emph{danger of neglecting other important ethical aspects} (e.g., ``Proportionality and Do No Harm'' is listed as the first principle before ``Fairness'' in UNESCO’s ``Recommendation on the
Ethics of Artificial Intelligence'', indicating its importance).   

\noindent\textbf{Challenge 3: Lack of systematic testing strategies.} Traditional systematic testing approaches are usually designed based on a coverage criteria where the goal is to cover the designated criteria as much as possible. Meanwhile, the closest testing approaches to ethics testing is fairness testing~\cite{galhotra2017fairness}. However, fairness testing focuses on testing group discrimination (e.g., female versus male) whereas each ethical problem can be manifested in multiple dimensions rather than simply two or more groups. For example, online harmful content can be manifested in the form of (1) hate and harassment (doxing, identity attack, identity
misrepresentation, insult, sexual aggression, and
threat of violence), (2) self-inflicted harm (eating disorder promotion and self-harm), (3) ideological harm (extremism, terrorism and organized crime
and misinformation), and (4) exploitation (adult sexual services, child
sexual abuse material, and scams) according to a unified taxonomy of harmful content~\cite{banko2020unified}. The search space for identifying harmful content is enormous, and yet identifying each type of harmful behavior in automatically generated content is important to the society, especially with the increasing reliance on GAI. 

\section{Definition of Ethics Testing}
\label{sec:defini}

We introduce two simplified assumptions of generative AI systems before presenting the formal definition of ethics testing. First, we define generative systems $Sys$
as a black box that maps textual inputs (usually written in natural languages and/or software programs as \emph{prompts}) to a pair of outputs ($stat, cont$) where $stat$ represents the outcome (success or failure) of running the generative system $Sys$ on the given input\footnote{$stat$ may not be explicitly stated but be implicitly inferred from the output when there is a successful outcome.}, whereas $cont$ denotes the generated content by $Sys$ (which could be empty if the generative system refuses to generate any content). Although some generative AI systems may be more complex (e.g., multi-modal systems that also accept images as input), this simplified assumption is sufficient for the
purposes of ethics testing: All other forms of inputs, user actions and environmental variables can be modeled or translated to textual inputs, and the generated outputs (including warning message and generated content) can be modeled as a pair of outputs where the exit status of the system denotes the $outcome$ and other outputs (e.g., the warning message) are concatenated as parts of generated content $content$. %When software has multiple output characteristics,  with respect to each output characteristic separately. 
The definitions can be extended to
multiple inputs without significant conceptual reformulation.  

Second, we assume that an unethical input can be obtained by starting with an ethical input and applying certain transformations. Thus, to test a generative system's robustness against unethical inputs, we start with ethical inputs and apply a set of transformations to obtain unethical content as the test inputs. Our assumption is inspired by Mencius's~\cite{hu2023confucian} and Aristotle's theory of innate human goodness~\cite{yu2001moral}: human behaviors are benign at the beginning and then unethical behaviors are derived from them.
%we assume that \emph{the input to a generative systems is naturally good} (i.e., the input is ethical to begin with). %and  the output characteristic are categorical variables, each having a set of possible values (e.g., race, gender, eye color, age ranges, incomeranges). 
This assumption also aligns well with the 
Competent Programmer Hypothesis in mutation analysis that ``the version of program produced by a competent programmer is close to the final correct version of a program''~\cite{gopinath2014mutant,budd1979mutation} (in ethics testing, an ethical behavior is ``correct'' in the ethical perspective).
This assumption allows us to design a set of rules that can induce unethical behavior into the input to $Sys$, %\todo{to check if the unethical behavior is added into the input or $Sys$; if it is added to the input, then it violates the assumption that the input is ethical?}, 
and simplifies our checking of the expected outputs. 

%simplifies our measure of causality. 
%TODO: I still need to write this part

\begin{definition}[Ethics Testing]
\label{def:ethicstesting}
Given a input prompt $inp$ to a generative system $Sys$ where $inp$ is innately ethical, \textbf{ethics testing} applies a set of transformation rules into $inp$ that aim to induce unethical behavior in $Sys$, to test $Sys$'s robustness against generating %leading $Sys$ to possibly generate
unethical content represented by $out$. The outcome $stat$ of the system $Sys$ is represented by a binary variable where $true$ corresponds to the case where $Sys$ successfully generates an output $out$ and $false$ means that the system $Sys$ refuses to generate any content $out$ (except for a warning message where $out$ denotes the warning message). 
\end{definition}

Compared to the prior definition of fairness testing~\cite{galhotra2017fairness} that focuses on group discrimination, Definition~\ref{def:ethicstesting} has two key differences: (1) it imposes a  stricter rule by taking into special consideration the outcome of generative systems because it is important to distinguish whether unethical content has been generated or not (our intuition is that a testing framework should check whether a generative system has violated ethical principles by generating unethical content, considering the fact that users can potentially misuse the generated content as soon as the content has been produced); and (2) an unethical behavior is defined and guarded by an ethical principle (e.g., the ``Do no harm'' principle) instead of whether it belongs to a different group (e.g. race, gender) as in fairness testing.






\section{A framework for ethics testing}
\label{sec:frame}

We propose a draft overview of our testing framework for ethics testing.
Figure~\ref{overview} shows an overview of our testing framework. 

\subsection{\modify{Dataset Construction.}}\label{dataset}
The first key component of the framework is a dataset that contains a collection of unethical keywords representing different types of unethical content as the ``vocabulary'' for performing subsequent testing. During prompt construction, the keywords will be injected into the prompt via transformations (e.g., rename the method into ``genocide'' where ``rename the method'' is a program transformation and ``genocide'' is the unethical keyword). %\heng{how about ``operators'' (how to apply a keyword) instead of ``keywords''?}.
We will form our vocabulary based on several sources: (1) unified taxonomy of harmful content~\cite{banko2020unified}, (2) our previous study of unethical behavior~\cite{win2023towards}, and (3) interview with researchers in ethics. \modify{Specifically, for each of the subcategories of harms in the unified taxonomy of harmful content~\cite{banko2020unified} (i.e., there are in total 13 subcategories), we will identify \emph{k} keywords representing each subcategory, leading to 13*k initial set of keywords. Then, we will augment the initial set of keywords with additional keywords from our previous study of unethical behavior~\cite{win2023towards} (e.g., genocide) to obtain words representing the terms used by open-source communities. As some keywords can be representing technical terms specific to generative AI, we will further conduct interview with researchers in ethics to obtain more technical terms that are unethical (e.g., ``AI slop'' that represents low quality media ).} Given the set of unethical keywords, we will design a set of code and non-code transformations for injecting the unethical keywords into the prompt. Then, the constructed prompts will be given to code-based and non-code-based (e.g., image generation and natural language generation) generative AI systems.  

%\todo{Haibo: add the figure}. Our   

\begin{figure}[H]
        \centering
\includegraphics[width=\textwidth]{workflow.png}
        \caption{An draft overview of our testing framework\Description[<short description>]{An draft overview of our testing framework}.} %\heng{shall we add the prompt inputs in parallel to the unethical keywords dataset?} \heng{maybe also add a component at the end to verify the output of the GAI systems?}}
        \label{overview}
\end{figure}

%mostly focus on fairness




%As a result of the recent interest in automatic programming, the set of problems associated with automatically generated code have received wide attention.In this article, we thus examine how trust boundaries can shift when we integrate automatically generated code into a software project. One of the technical questions that could be of interest for the research community are the acceptability criterion for integrating LLM generated code into a software project.


%The capability of LLMs augmented by program analysis tools in automating key programming tasks such as bug-fixes and feature additions, as articulated in the recently proposed SWEbench \cite{swe} is also worthy of study. The last mile improvement of automatically generated code from LLMs, through the systematic use of program repair \cite{fan2023automated} remains a possibility to explore~\cite{liu2023automated}. Such a penultimate auto-repair strategy can help provide specific evidence of correctness (such as passing curated tests) that builds confidence towards accepting LLM-generated code into a code repository. 

%We also study the impact of LLMs in automating non-code artifacts and processes such as test generation, code review and code summarisation. More importantly from the human-LLM interaction perspective, we seek to provide an emerging new outlook in future day programming. Traditionally, when formal specifications are unavailable, software engineers have resorted to {\em program comprehension} or specification inference to understand the functionality of a complex software system. This practice is particularly relevant when the software system is not built as a monolithic  artifact, but rather assembled via the co-operation of different teams or via open-source contributions. 

%We note that the traditional program comprehension problem is conducted by the human, and may involve the usage of analysis / debugging tools to understand the working of a complex software system. In the age of LLM driven programming, we could postulate a {\em new ethics testing problem} - where based on the natural language requirements LLMs augmented by program analysis tools can automate bulk of the comprehension tasks. There could be structured provisions for consulting the human to disambiguate requirements, at different stages of the comprehension process. Studying the mechanisms for such human-LLM collaboration and providing adequate primitives for consulting the human programmer by the LLM / analyzers could point us to the programming environments of the near future. We also underline the possibility of automated program repair of automatically generated code as a flexible mechanism for trusted automatic programming. These could feature in future day programming environments of 2030-35 and beyond.


==> sec4-future.tex <==



\section{Future: Programming environment of 2030-35 and beyond}

%{\bf\em Writer: Abhik Roychoudhury, Shin Hwei Tan}


In the programming environment of 2030-35 where LLM-based auto-programming techniques have reached certain level of maturity, programmers may need to switch to different roles to fully utilize the power of auto-programming.

\begin{figure}
        \centering

\begin{tabular}{cc}
\begin{tabular}{c}
        \includegraphics[width =0.35\textwidth]{picture-composer.jpg}
\end{tabular} &
\begin{tabular}{c}
\includegraphics[width=0.35\textwidth]{qa.jpg}
\end{tabular}\\
(a) & (b) \\
\end{tabular}
        \caption{Evolution of programmer roles captured by DALL-E;
        programmer role (a) as code composer and designer instead of code writer, 
        (b) as quality assurance specialist instead of code writer.
        }\label{combined}
    \end{figure}

%\noindent\textbf{Adaptive selection of LLMs for various downstream tasks.} 
\paragraph*{Programmer as code composer and designer instead of code writer.} With the advancement of LLM-based auto-programming, many software maintenance tasks that require code writing can be automatically solved by invoking the appropriate LLMs. Figure~\ref{combined}(a) shows an AI-generated picture by Image Creator that uses DALL·E where programmers acts as code composer and designer instead of code writer. Instead of playing the traditional role of a programmer who meticulously writes code for solving different tasks, they can focus on tasks that require high-level understanding of the requirements (e.g., designing the overall structure of the program and tentative algorithms), allowing automated tools to select the most effective model for the relevant maintenance tasks in which relevant code will be automatically generated. As current techniques mainly focus on specializing LLMs for a specific downstream task of auto-coding (e.g., program repair, log statement, test generation) to improve the effectiveness for the given task, a future programming environment will intelligently predict and select the appropriate model to invoke based the context of the downstream task. There are two scenarios in which LLM-based auto-programming can change the future programming environment: (1) in an Integrated Development Environment (IDE) setting, (2) in a continuous integration (CI) workflow. For example, in the IDE setting that requires instant feedback from the auto-coding tool for efficient interaction, future techniques can design a lightweight tool that can automatically complete and suggest relevant code snippets based on the (1) current surrounding code and (2) the list of available tasks (e.g., suggest adding a JUnit test for the newly written Java method or adding a log statement before a graceful exit of a program).  Meanwhile, in a CI workflow, certain event that represents abnormal behavior of a software system (e.g., test failures, build failures) can automatically trigger the need for a software maintenance task (e.g., the need for a repair can be triggered after a test failure). In this scenario, more sophisticated techniques can be used to further confirm the validity of the trigger (e.g., to distinguish between test failure or flaky test). These techniques include program analysis techniques (such as symbolic execution), test generation techniques (based on code changes within a commit), and log analysis (program monitoring). 

 
\begin{figure}
        \centering
    \includegraphics[width=0.65\textwidth]{./figures/Lastmile.pdf}
        \vspace*{-0.05in}
        \caption{Automated repair of auto-generated code}\label{lastmile}
    \end{figure}
\vspace*{-0.05in}
\paragraph*{Programmer as quality assurance specialist.} Although many tasks can be automated, we foresee that concerns regarding the quality of the autogenerated code still remain. As some of the autogenerated code can be misaligned with the intention of the programmer, the programmer will need to play the role of a quality assurance specialist and spend more time in checking the validity of the generated code. Apart from using traditional testing and static analysis tools, more specialized automated program repair techniques can be designed (e.g., by referring to prior study~\cite{fan2023automated} that investigated the mistakes of auto-generated code) to reduce the time and effort involving in checking the quality of auto-generated code.  Figure~\ref{combined}(b) shows an AI-generated picture for programmer main role as quality assurance specialist.
Figure \ref{lastmile} shows a schematic that concretizes this last-mile improvement of autogenerated code $P$ produced from natural language description using a tool like Copilot. The autogenerated code may be subject to program repair guided by a given test suite $T$. However, the process of repair inspects or examines (either explicitly or implicitly) a domain of program edits --- trying to shrink the space of candidate edits which are suitable for improving program $P$. In this way, a repaired program $P'$ is generated from $P$. In the process of examining the domain of program edits (and presumably ruling out a lot of candidate edits), the program repair process generates many additional tests $T'$ over and above the test suite $T$ which was used to guide the program repair process. The oracle (or expected behavior) of these additional tests $T'$ can be obtained via some processing of the natural language description from which $P$ is derived.   The additional test inputs $T'$ (along with their oracles) can then serve as evidence of "correctness" of the repaired program $P'$.  We envision that code-generators of the future will not be only LLMs, but  LLM agents augmented with program analysis / repair capabilities. These augmented code generators may then try to commit code like human programmers, while submitting evidence in the form of generated tests $T'$ as evidence of correctness of (LLM-induced) code commits.  

\vspace*{-0.05in}
\paragraph*{Programmer-assisted safe auto-coding} %As there are prior incidents where using LLMs for auto-programming lead to leakage of sensitive data, programmers who would like to benefit from the power of LLM-based auto-programming will need to identify (and protect) the sensitive data before feeding them to LLMs. Existing code obfuscation techniques and data encryption algorithms can be used as a first layer of protection. %Figure~\ref{composer} shows an AI-generated picture for programmer-assisted automated programming. 
We envision that Large Language Model (LLM) generated code may be integrated into legacy code-bases of existing software projects. This could be in the form of libraries performing specific tasks, where the library code is generated with LLM. For safe integration of such LLM generated code in human-written software projects, one may need {\em sanitizer code} (e.g. \cite{asan}) so that the LLM generated code can be used by the bigger software project safely. Until we reach the stage of completely automating the generation of entire software projects, there may be a need to study (a) automated repair or improvement of LLM generated code, or (b) executing LLM generated code in a {\em contained} manner so that it can cause limited harm to the rest of the software system, or (c) generate verified LLM code whenever appropriate formal specifications are available. One first step towards verified LLM code can be to generate code in a programming language supporting verification ({\em e.g.}, see \cite{Misu24}). We could also generate both programs and proofs (about the program satisfying some formal properties) from LLMs. Such formal properties may be obtained from natural language, in which there is some work \cite{Mauro}. Automated generation of proofs from LLMs has also been recently studied \cite{Baldur}. All of these works provide impetus in moving towards higher assurance code from LLMs. 

\vspace*{-0.05in}
\paragraph*{Autonomous Program Improvement} We view the approach of program repair on unsafe code generated by LLMs to be a more {\em flexible} approach for automatically generating safe code (as it is based on code transformations), as compared to tuning or restriction of LLMs to generate safe outputs. Moving forward, researchers can examine this line of work, in addition to significant short-term efforts in prompt engineering and LLM tuning. Repair of the automatically generated code based on tests gives us more flexibility, partly because we can also choose the tests we use to guide the program repair. The repair as well as other tasks like feature addition can be achieved autonomously by LLM agents which are aware of the structure of the code. The recent work on AutoCodeRover \cite{acr} is an example work in this direction. In the near future, the focus will be to improve the efficacy of these agents. The combination of auto-coding from  natural language and autonomous software improvement using LLMs, is an enticing possibility which can be achieved by 2030. This would shift the role of a future software engineer towards achieving {\em assured autonomy} by focusing on {\em trust} of the autonomous artifacts, instead of engineering software systems at {\em scale}. The scale of software systems is likely to be achieved automatically in future, thus shifting the attention to \underline{\em trust}.

%If the LLM-generated code is subject to test generation (with test oracles derived from natural language descriptions), the tests can pinpoint errors which are then used to drive program repair. This workflow can be developed  on top of recent works like AutoCodeRover \cite{acr}.

%\vspace*{-0.05in}
\paragraph*{Looking even further} Autonomous improvement of automatically generated code need not be restricted to application level programming. We could examine the feasibility of automatically repairing probabilistic programs, which are generated automatically. Probabilistic  programming succinctly expresses statistical inference tasks on probabilistic models \cite{fose14}, and are supported in the back-end by machine learning frameworks like Pytorch \cite{pytorch}. Recently symbolic execution of probabilistic programs was proposed \cite{Voogd23} which raises the possibility of semantics-aware probabilistic program repair, after an initial LLM guided automated generation of  probabilistic program snippets. This line of work could help us progress towards automated self improvement of learning tasks,  a speculative direction of future research.


%\begin{figure}
%        \centering
%        \includegraphics[width =0.35\textwidth]{collaboraterobot.jpg}
%        \caption{Programmer-assisted safe automated programming}\label{composer}
%    \end{figure}

%\noindent\textbf{Integrating auto-generated code into human-written code?} TODO : % legacy code

%- maybe move to the last mile improvement\noindent\textbf{Program Comprehension aided by programming environment?} TODO: adding a new feature or bug fix to understand code/ for software evolution with help of program analysis

%-maybe move to the explanability section


